GPU-enabled Function-as-a-Service for Machine Learning Inference

Function-as-a-Service (FaaS) is emerging as an important cloud computing service model as it can improve the scalability and usability of a wide range of applications, especially Machine-Learning (ML) inference tasks that require scalable resources and complex software configurations. These inference tasks heavily rely on GPUs to achieve high performance; however, support for GPUs is currently lacking in the existing FaaS solutions. The unique event-triggered and short-lived nature of functions poses new challenges to enabling GPUs on FaaS, which must consider the overhead of transferring data (e.g., ML model parameters and inputs/outputs) between GPU and host memory. This paper proposes a novel GPU-enabled FaaS solution that enables ML inference functions to efficiently utilize GPUs to accelerate their computations. First, it extends existing FaaS frameworks such as OpenFaaS to support the scheduling and execution of functions across GPUs in a FaaS cluster. Second, it provides caching of ML models in GPU memory to improve the performance of model inference functions and global management of GPU memories to improve cache utilization. Third, it offers co-designed GPU function scheduling and cache management to optimize the performance of ML inference functions. Specifically, the paper proposes locality-aware scheduling, which maximizes the utilization of both GPU memory for cache hits and GPU cores for parallel processing. A thorough evaluation based on real-world traces and ML models shows that the proposed GPU-enabled FaaS works well for ML inference tasks, and the proposed locality-aware scheduler achieves a speedup of 48x compared to the default, load balancing only schedulers.

==> cover.tex <==
We thank all the anonymous reviewers for the constructive comments. In this revision we have addressed these comments as follows. All major changes are colored in red in the paper.

\vspace{6pt}
\noindent \textbf{Review 1:}

\begin{itemize}
    \item Explained the storage setup of the testbed in Section V.A. 
    \item Removed the imprecise statements pointed out by the reviewer.
    \item Added discussions of related works (Triton, funcX) in Section II.A and Section II.C.
    \item Cleaned up Algorithms 1 and 2 and improved their clarity.
\end{itemize}

\vspace{6pt}
\noindent \textbf{Review 2:}

\begin{itemize}
    \item Added discussions of related model serving systems (TensorFlow Serving, Triton, TorchServ) and explained how our work advances the state of the art in Section II.C.
    \item Added a new Section VI to discuss security, usability, and support of heterogeneous GPUs. 
    \item Explained how our solution supports different (versions of) machine learning frameworks in Section VI.
\end{itemize}

\vspace{6pt}
\noindent \textbf{Review 3:}

\begin{itemize}
    \item Added discussions of related GPU-based model training works (CROSSBOW, Antman) in Section II.C and related GPU sharing works (KubeShare, AWS virtual GPU plugin, MPS) in Section II.D, and explained how our work advances the state of the art.
    \item Added the discussion of scalability and security in the new Section VI Discussions. 
    \item Explained the support of different cache replacement policies in Section VI.
\end{itemize}

\vspace{6pt}
\noindent \textbf{Review 4:}

\begin{itemize}
    \item Added the discussion of scalability in the new Section VI Discussions. 
    \item Added discussions of related model serving solutions in Section II.C.
    \item Improved Fig. 5 and 6 as suggested.
\end{itemize}
